Towards an Awareness of Time Series Anomaly Detection Models' Adversarial Vulnerability

Time series anomaly detection is extensively studied in statistics, economics, and computer science. Over the years, numerous methods have been proposed for time series anomaly detection using deep learning-based methods. Many of these methods demonstrate state-of-the-art performance on benchmark datasets, giving the false impression that these systems are robust and deployable in many practical and industrial real-world scenarios. In this paper, we demonstrate that the performance of state-of-the-art anomaly detection methods is degraded substantially by adding only small adversarial perturbations to the sensor data. We use different scoring metrics such as prediction errors, anomaly, and classification scores over several public and private datasets ranging from aerospace applications, server machines, to cyber-physical systems in power plants. Under well-known adversarial attacks from Fast Gradient Sign Method (FGSM) and Projected Gradient Descent (PGD) methods, we demonstrate that state-of-the-art deep neural networks (DNNs) and graph neural networks (GNNs) methods, which claim to be robust against anomalies and have been possibly integrated in real-life systems, have their performance drop to as low as 0%. To the best of our understanding, we demonstrate, for the first time, the vulnerabilities of anomaly detection systems against adversarial attacks. The overarching goal of this research is to raise awareness towards the adversarial vulnerabilities of time series anomaly detectors.

==> sections/1_introduction.tex <==






\vspace{-10pt}
\section{Introduction}

\label{sec:intro}
% \hl{talk about anomaly as unsupervised task and intrusion as supervised task but clarify why.}
Machine learning and deep learning have profoundly impacted numerous fields of research and society over the last decade~\citep{SAM1,goodfellow2016deep}. Medical imaging~\citep{MedicalImagingSurvey}, speech recognition~\citep{SpeechRecognitionSurvey}, environmental sciences~\cite{zeb1,zeb2} and smart manufacturing systems~\citep{SmartManufacturingSurvey} are a few of these areas. With the proliferation of smart sensors, massive advances in data collection and storage, and the ease with which data analytics and predictive modeling can be applied, multivariate time series data obtained from collections of sensors can be analyzed to identify 
particular patterns that can be interpreted and exploited. Numerous researchers have been interested in time series anomaly detection~\citep{AnomalySurvey,CLMPPCA,ITAD,YJ1,Shah_KDD_workshop,Anomaly_simon1,Anomaly_simon2,Anomaly_simon3}. For instance, time series anomaly detection methods are used in the aerospace industry for satellite health monitoring~\citep{CLMPPCA,ITAD,OmniAnomaly}. %, while intrusion detection methods are employed in the \hl{computer networking/security and} automobile industry for \hl{variety of computer networks as well as} in-vehicle controller area networks. 
These deep neural network-based solutions outperform the competition on a variety of benchmark datasets. However, as deep learning became more prevalent, researchers began to investigate the vulnerability of deep neural networks, particularly to adversarial attacks. In the context of image recognition, an adversarial attack entails modifying an original image in such a way that the modifications are nearly imperceptible to the human eye~\citep{Fawaz14}. The modified image is referred to as an adversarial image, as it will be classified incorrectly by the neural network, whereas the original image will be classified correctly. One of the most well-known real-world attacks involves manipulating the image of a traffic sign in such a way that it is misinterpreted by an autonomous vehicle~\citep{Fawaz15}. The most common type of attack is gradient-based, in which the attacker modifies the image in the direction of the gradient of the loss function relative to the input image, thereby increasing the rate of misclassification~\citep{Fawaz14,FGSM,PGD}. 


% \begin{wrapfigure}{r}{0.5\textwidth}
%   \begin{center}
%     \includegraphics[width=0.5\textwidth]{figures/RealvsAdv.pdf}
%     \includegraphics[width=0.5\textwidth]{figures/RealvsAdv_error.pdf}
%   \end{center}
%   \caption{Example of ground truth and perturbed time series using FGSM and PGD attacks on CLMPPCA.}
%   \label{fig:clmppca}
% \end{wrapfigure}

While adversarial attacks have been extensively studied in the context of computer vision areas, they have not been extensively investigated for anomaly detection systems with time-series data. It is surprising to see much less research performed, given the increasing popularity of deep learning models for classifying time series~\citep{Fawaz2,Fawaz9,Fawaz19}. Additionally, adversarial attacks are possible in a large number of applications that require the use of time series data. 
For instance, Figure~\ref{fig:clmppca} (top) depicts the original and perturbed time series for the Korean Aerospace Research Institute's KOMPSAT-5 satellite (KARI)~\cite{CLMPPCA}. % \simon{add citation for data source and paper}.
The prediction error (see Figure~\ref{fig:clmppca}, right) is generated by the Convolutional LSTM with Mixtures of Probabilistic Principal Component Analyzers (CLMPPCA) method~\cite{CLMPPCA}, which is currently incorporated at KARI, to predict anomalies. While CLMPPCA accurately predicts the anomaly for the original time series, adding small perturbations in the form of FGSM and PGD attacks causes the entire input samples to be classified as an anomaly. This attack can have a severe impact on the satellite health monitoring.

We present, transfer, and apply adversarial attacks that have been demonstrated to work well on images to time series data (containing anomalies) in this work. Additionally, we present an experimental study utilizing benchmark datasets from the aerospace and power plant industries and server machines, demonstrating that state-of-the-art anomaly detection methods are vulnerable to adversarial attacks. We highlight specific real-world use cases to emphasize the critical nature of such attacks in real-world scenarios. Our key findings indicate that deep networks for time series data, similar to their computer vision counterparts, are vulnerable to adversarial attacks. As a result, this paper emphasizes the importance of protecting against such attacks, particularly when anomaly detection systems are used in sensitive industries such as aerospace and power plants. 
% Additionally, we demonstrate that adversarial time series learned using one network architecture can be transferred to another (\hl{see Appendix X}).
Finally, we discuss some mechanisms for avoiding these attacks while strengthening the models' resistance to adversarial examples.

\textbf{Aim, Scope and Contribution. } 
In this work, we do not propose any novel adversarial attack method. However, we apply and demonstrate the threat of well-known existing adversarial attacks such as FGSM and PGD towards state-of-the-art anomaly detection methods for multivariate time-series data. In comparison to the computer vision domain, where adversarial attack has been extensively studied and investigated, the literature on novelty detection, and particularly on anomaly detection, is noticeably devoid of such studies. The purpose of this paper is to bring attention to this critical issue, whereas 
%\hl{whereas ...} \simon{emphasize one more time}
time series anomaly detection models also play pivotal roles in real-world scenarios as other vision tasks. Additionally, we hope to encourage researchers to consider robustness to adversarial attacks when evaluating time-series based future detectors. The paper's scope was limited to analyzing SOTA anomaly detectors. % (Note: As intrusion detection is a vast domain we consider only one sub-domain i.e., intrusion detection in Controller Area Network).
% Finally, to demonstrate that the current generation of anomaly detectors are unprepared against adversarial attacks, \sh{We successfully applied adversarial attacks on a deployed systems in the power plant and aerospace industry.} %\simon{unclear sentence...}
Finally, we successfully degraded the detection performance of deployed systems in the power plant and aerospace industries by employing adversarial attacks. It highlights how vulnerable the current generation of anomaly detectors is to adversarial attacks. Our source code and other implementation details are available here:   {\small \color{RoyalBlue}\url{https://github.com/shahroztariq/Adversarial-Attacks-on-Timeseries}}.



% Main Contributions
% Attacks are not news.
% But demonstrate they are vulnerable…

% No new attacks…we have to defend…
% You need Eq. 


% Novelty: 
% 1. though classification, no one adv attack on time series/regression (anomaly or outlier detection) model. 

%       0) Generate adv examples/samples for time series w/ popular methods: math

% Show the vulnerabilities of the famous (multiple or different types of DNN architecture) deep learning-based anomaly detection/outlier algorithms (high performing (LSTM, ConvLSTM, GNNs) DNN algorithms are easily deceived, fooled or very easy to create the adversarial attacks.): math

%  Comprehensive  evaluate and analyze using different kinds of performance metrics 
% over different public and private datasets (datasets: patterns/flavors are different): Aerospace applications (KARI+), car applications, UCR, SMD dataset, CPS

% Threat (attacker) model: We assume the whitebox attack model, where attacker or faulty sensor can inject (adding carefully crafted malicious noise) the +/- noise to ML model.  

% Conclusion: More research on defense on adv. time series attack.


% 2. Adv. attack framework to test the robustness 
% Attack algorithms: FGSM. PGD, SparseL1descent
% Prediction/Regression Algorithms: MSCRED, GNN (ML4ITS), attack ours (ConvLSTM) 
% DataSet: UCR, SMAP, MSL, etc…
% Threat models (we can think of)


% \blindtext


% \Blindtext







\begin{figure}[t]
\centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/RealvsAdv.pdf}
        % \caption{}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/RealvsAdv_error.pdf}
        % \caption{}
    \end{subfigure}%\hfill
    \vspace{-10pt}
    \caption{Example of ground truth and perturbed time series using FGSM and PGD attacks on CLMPPCA.}
  \label{fig:clmppca}
  \vspace{-20pt}
\end{figure}


==> sections/2_related.tex <==
% \vspace{-10pt}
\section{Related Work}
\label{sec:related}
In this section, we present background information, notations, and related works, with a particular emphasis on time series anomaly detection and adversarial attacks. 
% https://arxiv.org/pdf/2009.11911.pdf

% https://arxiv.org/abs/1802.03041

% https://www.ijcai.org/proceedings/2020/0173.pdf
\noindent
\textbf{Background and Notations. } When performing a supervised learning task, we define $D= \{(s_i,y_i)|i=1,\dots,N\}$ to represent a dataset containing N data samples. Each data sample is composed of a $m$-dimensional multivariate time series $s_i$ and a single target value $y_i$ for classification. However, the majority of anomaly detection occurs in an unsupervised setting. As a result, we take a slightly different approach from the supervised task. 
%We will observe such formation in intrusion detection scenarios (see Section~\ref{sec:intrusion_baselines}). 
Hence, for unsupervised learning, each data sample is again composed of a $m$-dimensional multivariate time series $s_i$ however, $y_i$ is an $n$-dimensional multivariate time series obtained from an autoregressive model, predicting the future. In most cases, $n=m$ however, they can be different as well. Moreover, we define any deep learning method as
$\mathcal{F} (\cdot) \in \displaystyle f: \R^N \rightarrow \widehat{y}$
% $f(\cdot)\in \mathcal{F}:\displaystyle \R^N \to \widehat y$
and loss function (e.g., cross entropy or mean squared error) as $\mathcal{L}_f(\cdot\,,\cdot)$. Finally, generating an adversarial instance $s_i^{adv}$ can be described as an optimization problem given a trained deep learning model $\mathcal{F}$ and an original input time series $s_i$, as follows:
\begin{equation}
\small
\centering
% \begin{split}
% \;\;\;&
\min \left \| s_i-s_i^{adv}\right \| %\\
  \;s.t.\;
  \mathcal{F}(s_i)  =\widehat{y_i},\;\;% &
  \mathcal{F}(s_i^{adv})=\widehat{y^{adv}_i} \;\; and \;\; \widehat{y_i} \ne \widehat{y^{adv}_i}
% \end{split}
\end{equation}
% In the case of a supervised learning task, we let 
\noindent
\textbf{Adversarial Attacks.}
In 2014, \citet{Fawaz24} introduced adversarial examples against deep neural networks for image recognition tasks for the first time. Following these inspiring discoveries, an enormous amount of research has been devoted to generating, understanding, and preventing adversarial attacks on deep neural networks~\citep{Fawaz15,FGSM,PGD}. Adversarial attacks can be broadly classified into two types: White-box and Black-box attacks. As White-box attacks presume access to the model's design and parameters, they can attack the model effectively and efficiently using gradient information. By contrast, Black-box attacks do not require access to the output probabilities or even the label, making them more practical in real-world situations. However, Black-box attacks frequently take hundreds, if not millions, of model queries to calculate a single adversarial case.

The majority of adversarial attack techniques have been proposed for use in image recognition. For instance, a Fast Gradient Sign Method attack was developed by~\citet{FGSM} as a substitute for expensive optimization techniques~\citep{Fawaz24}.
%Madry \textit{et al.}
\citet{PGD} proposed Projected Gradient Descent (PGD) in response to the success of FGSM. PGD seeks to find the perturbation that maximizes a model's loss on a particular input over a specified number of iterations while keeping the perturbation's size below a specified value called epsilon ($\epsilon$). This constraint is typically expressed as the perturbation's $\normltwo$ or $\normmax$ norm. It is added to ensure that the content of the adversarial example is identical to that of the unperturbed sample — or even to ensure that the adversarial example is imperceptibly different from the unperturbed sample. Carlini-Wagner is another well-known attack \citep{CarliniWagnerL2}. However, it is primarily intended for $\normltwo$ norm-based attacks, whereas this study focuses exclusively on $\normmax$ norm-based attacks.

\noindent
\textbf{Adversarial Attacks on Time Series Anomaly Detectors. } 
Surprisingly, limited efforts have been made to extend computer vision-based adversarial attacks to time series anomaly detection domain. % Surprisingly, the community has ignored adversarial attack approaches for time series anomaly detection tasks.
However, a few adversarial attack approaches have been proposed recently for the time series classification task, which are tangentially related to our work.
For instance, in their work on adopting a soft K Nearest Neighbors (KNN) classifier with Dynamic Time Warping (DTW), \citet{Fawaz26} demonstrated that adversarial examples could trick the proposed nearest neighbors classifier on a single simulated synthetic control dataset from the UCR archive~\citep{UCR}. Given that the KNN classifier is no longer considered the state-of-the-art classifier for time series data~\citep{fawaz27}, \citet{FawazADV} extend this work by examining the effect of adversarial attack on the more recent and commonly used ResNet classifier~\citep{ResNet}. \citet{FawazADV}, on the other hand, focused mainly on univariate datasets from the UCR repository. As a result, \citet{HarfordAdv} investigate the influence of adversarial attacks on multivariate time series classification using the multivariate dataset from UEA repository~\citep{UEA}. However, \citet{HarfordAdv} only consider basic methods such as 1-Nearest Neighbor Dynamic Time Warping~\citep{1NNDTW} (1-NN DTW) and a Fully Convolutional Network (FCN). \citet{fazle} and \citet{HarfordAdv} attacked models using Gradient Adversarial Transformation Networks (GATNs). %Because they also evaluated non-differentiable classical time series models, they employed a knowledge distillation strategy to train a student network that replicated the original classifier's predictions. As a result,
However, they examined just transfer attacks, a relatively weak sort of Black-box attack. Only \citet{Siddiqui} demonstrated the effectiveness of gradient-based adversarial attacks on time series classification and regression networks. However, they considered a very simple baseline for the attack, containing only 3 convolutional, 2 max-pooling, and 1 dense layer.


 
%However, recently, adversarial attack method have been proposed for the time series classification task, which in-directly related to our problem. 



\textbf{\textit{Note}: } Our study differs from previous research in that we focus on time series anomaly detection rather than the broader classification problem. More precisely, we explore autoregressive models that have been mostly overlooked in prior works. Additionally, rather than targeting generic deep neural networks KNN with DTW or ResNet, we investigate state-of-the-art anomaly detection methods. For instance, when it comes to anomaly detection, we focus on the most contemporary and commonly used techniques, such as MSCRED~\citep{MSCRED}, CLMPPCA~\cite{CLMPPCA}, and MTAD-GAT~\cite{MTADGAT}.
%Similarly, for controller area network intrusion detection, we explore two well-known methods: CAN-ADF~\citep{CANADF} and CANTransfer~\citep{CanTransfer}.
Section~\ref{sec:exp} will cover these methods in further depth.

% \Blindtext

==> sections/3_Methodology.tex <==
% \section{Methodology}
% \label{sec:method}

\begin{figure*}
    \centering
    \includegraphics[%trim={20pt 19pt 24pt 18pt},clip,
    width=1\linewidth]{"figures/Adv_ICLR-Pipeline".pdf}
    \vspace{-25pt}
    \caption{Pipeline of a typical time series anomaly detection's training phase and our  adversarial attack phase. }
    \label{fig:pipeline}
    \vspace{-10pt}
\end{figure*}

\vspace{-10pt}
\section{Threat Model}
\label{sec:method}
To fully define the adversary, we divide the threat model into three subsections based on the adversary's capabilities, knowledge, and goals.

\noindent
\textbf{Adversary's Capabilities. }
We consider an adversary whose objective is to reduce the effectiveness of a victim model.  The attacker can apply the perturbations by modifying the victim's test-time samples, for example, by compromising a sensor or the data link that collects the data for inference. We investigate a $\normmax$ norm threat model with a $0.1$ epsilon. Due to the variable input range of time series data, there are no box constraints, in contrast to the visual image, where the pixels take on a definite value between $[0, 255]$. As a result, the data was standardized in our case using a zero-mean and unit standard deviation which justified the choice of $0.1$ as the epsilon value. 

% \hl{
% 1. According to 1 reviewer,  the attacker is very strong we need to update the threat model with more realistic assumptions as the system we focus in this work are considered as deployed methods.

% 2. Reviewer mentions that these systems must be behind some security walls. Which we should explain how the attacker will bypass.
% } \simon{I can add} 

% \simon{
% Previously, we used white box. But now we will add black box as well by transferring adversarial attacks from a different backbone method}


\noindent
\textbf{Adversary's Knowledge. }
To evaluate the vulnerability of anomaly detection systems, we examine non-targeted White-box and Black-box scenarios. Typically, the attacker is given complete knowledge of the victim model, including its training data and the model's tunable parameters and weights.  However, we believe it to be unpractical in our scenario. As most of the system in our analysis are behind some layer of firewall or defense protection and most of the model parameters are hidden. Therefore, we consider two  types of adversary's knowledge as follows: 

% \noindent
\textbf{1) \textit{Complete Knowledge}: } The attacker understands how the model and its parameters works.  We can consider a \textit{White-box} attack to be the most appropriate method for this type of adversary. 

\textbf{2) \textit{Partial or No Knowledge}: } Given that the attacker has no or limited knowledge of the system, a \textit{Black-box} attack is the most appropriate method in this case. As a result, strategies such as transfer-based priors~\citep{TransferPrior} can be applied by the adversary.
% Additionally, in Appendix \hl{X}, we examine Black-box scenarios, in which the attacker creates $s_i^{adv}$ using a surrogate model and applies it to an unknown victim model. \hl{might add if i have results}

\noindent
\textbf{Adversary's Goals. } 
The adversary considers two cases: (i) normal to anomaly and (ii) anomaly to normal. In (i), the adversary creates a $s_i^{adv}$ for each test sample $s_i$ so that the models interpret it as an anomaly, thereby generating a false-positive. However, in (ii), the adversary fabricates $s_i^{adv}$ to achieve the inverse effect, namely, to cause the model to predict an anomaly as normal, hence generating false-negative examples. As anomalies are rare events, even a few misclassifications caused by the adversary can have a detrimental effect on the model's performance.

\vspace{-5pt}
\section{Adversarial Attack Generation}
% \textbf{Fast Gradient Sign Method (FGSM) Attack. }
The Fast Gradient Sign Method (FGSM) attack was proposed for the first time by \citet{FGSM}. The training of neural networks entails minimizing a loss function by adjusting the network weights. FGSM, on the other hand, does the opposite by adjusting the input samples in the direction opposite to the loss function's minimum. Thus, the FGSM attack is concerned with the computation of optimal perturbation series $\eta$, which can be added/summed to an input sample pointwise (i.e., a point refers to a single timestep) in order to maximize the classification loss function, i.e., cause misclassifications. This is mathematically expressed as:
\begin{equation}
    \eta = \epsilon \cdot \text{sign}\left (\nabla_s\;\mathcal{L}_f(s_i,y_i)\right )
\end{equation}
where $\nabla_s$ denotes the derivative of the network's loss, $\mathcal{L}_f(\cdot\,,\cdot)$, with respect to each timestep in $s_i$ (calculated for an input datapoint $s_i$ and it's true output $y_i$). To control the magnitude of the perturbation (i.e., to keep it imperceptibly small), $\epsilon$ is used as a multiplier factor. After that, the perturbed sample $s_i^{adv}$ can be computed as $s_i+\eta$. Note that FGSM requires the attacker to compute the loss function gradient with respect to a given input, which may not be possible directly. Due to the fact that FGSM requires knowledge of the internal workings of the network it is therefore referred to as a White-box attack. However, a surrogate model can be used to simulate the target model. An FGSM attack can be applied to the surrogate to generate adversarial examples~\citep{Mubarak15}, allowing for the use of such White-box attacks in practical scenarios~\citep{Mubarak16}.

% Madry \textit{et. al} 
\citet{PGD} proposed a more robust adversarial attack called Projected Gradient Descent (PGD). This attack employs a multi-step procedure and a negative loss function. It overcomes the problem of network overfitting and the shortcomings of the FGSM attack. It is more robust than first-order network information-based FGSM, and it performs well under large-scale constraints. Gradient Descent is essentially identical to the Basic Iterative Method (BIM)~\citep{Mubarak16} or the Iterative FGSM (IFGSM)~\citep{IFGSM} attacks. The only difference is that PGD initializes the example at a random location within the ball of interest (determined by the $\normmax$ norm) and performs random restarts, whereas BIM initializes at the original location.%PGD iterate in $\normmax$-ball to determine the maximum loss.
\begin{equation}
\begin{split}
    s^{adv}_{i,t+1}=\Pi_{s+\delta}& \left (s^{adv}_{i,t} + \alpha\;\text{sign}(\nabla_s\mathcal{L}_f(s^{adv}_{i,t},y))\right)\\&\;\;\; s.t. \;\;\; 1\leq t \leq T
\end{split}
\end{equation}
\noindent
where $\delta$ is a nonempty compact topological space, $T$ is the total number of iterations,  and $\alpha$ is the control rate.
An illustration of the overall pipeline is provided in Figure~\ref{fig:pipeline}.

% \end{figure}

==> sections/4_Experiment.tex <==
% \vspace{-25pt}
\section{Experimental Setup}
\label{sec:exp}
This section contains information on the benchmark datasets, evaluation metrics, criteria for selecting baselines, and chosen baselines.

\noindent
\textbf{Datasets} For anomaly detection we employ three public datasets: (i) Mars Science Laboratory rover (MSL) \citep{SMAPMSL}, (ii) Soil Moisture Active Passive satellite (SMAP) \citep{SMAPMSL}, and (iii) Server Machine Dataset (SMD) \citep{OmniAnomaly}, as well as one private dataset: (vi) Korean Aerospace Research Institute KOMPSAT-5 satellite (KARI) \citep{CLMPPCA} and one synthetic dataset: (v) from the MSCRED paper \citep{MSCRED}.
%Intrusion detection was performed using the CAN Dataset for intrusion detection (OTIDS) \citep{OTIDS}.
The datasets were chosen based on our baselines' shown ability to provide state-of-the-art performance on them. %these datasets.
Table~\ref{tab:datasets} summarize these datasets.

\noindent
\textbf{Evaluation Metrics} %For intrusion detection, we use three metrics: Precision, Recall, and F1-score. However, we only provide the $F_1$ score in the main text (please refer to Appendix X for detailed results).
To obtain the final classification result for anomaly detection methods, we observed that the majority of detectors use a thresholding method on top of the neural network's predictions, which are expressed as an anomaly score or prediction error. The precision, recall, and F1-score are then calculated using the results from thresholding methods. While these metrics are beneficial, the true impact of the adversarial attack is visible primarily in anomaly detectors' anomaly score and prediction errors. Therefore, we include Figure~\ref{fig:clmppca}, \ref{fig:mtad-gat} and \ref{fig:mscred}, as illustrations of this impact. Additionally, we include more related figures in Appendix~\ref{app_sec:MSCRED}--~\ref{app_sec:CLMPPCA}.
% \usepackage{graphicx}
% \usepackage{booktabs}
\begin{table}[t!]
\centering
\caption{A summary of anomaly detection datasets.}
\label{tab:datasets}
\vspace{-10pt}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{lcccccc} 
\toprule
\textbf{Statistics} & \textbf{SMAP} & \textbf{MSL} & \textbf{SMD} & \textbf{KARI} & \textbf{Synthetic}\\ %& \textbf{OTIDS} \\ 
\hline
Dimensions & 55 & 27 & 28 & 4-35 & 30\\% & 11 \\
Anomalies & 13.13\% & 10.27\% & 4.16\% & 1.00\% & 1.10\% \\% & 48.64\% \\
Train Size & 135,183 & 58,317 & 708,405 & 4,405,636 & 8,000 \\% & 2,306,954 \\
Test Size & 427,617 & 73,729 & 708,420 & 17,622,546 & 10,000 \\ %& 2,306,955 \\
\bottomrule
\end{tabular}
}
\vspace{-15pt}
\end{table}


%We use three metrics i.e., Precision, Recall and F1-score for intrusion detection. 
% For anomaly detection methods, we observed that during post-processing most detector use a thresholding method on top of the neural network's predictions, which are in the form of anomaly score or prediction error, to get the final classification result. This result is then used to calculate  prediction, recall and F1-score. These metrics are useful however, the real impact of adversarial attack can be mainly be seen on the anomaly score and prediction errors of the anomaly detectors. Therefore, in Table X we also show these results. 
%However, we observe that different metrics are used to predict anomalies for different anomaly detection methods. 
%The most frequently used are anomaly scores and prediction errors.%, both of which are used in conjunction with a thresholding method. 
%As a result, we use one of these two metrics based on the baseline method for anomaly detection.% For intrusion detection, we use F1-score as the evaluation metrics. However, we find that for different anomaly detection methods different metrics are used to predict the anomalies. The most common ones are anomaly scores and prediction errors. Therefore, based on the baseline method we use one of these two metrics. 


 \vspace{-6pt}
\subsection{Anomaly Detection Baselines}
\subsubsection{\textbf{Selection Criteria}}
We conduct experiments on the following baselines to demonstrate that the vulnerability to adversarial attacks is common among several state-of-the-art anomaly detection architectures.
% \begin{itemize}[leftmargin=10pt]
    % \item \textit{Anomaly Detection Baselines}:
    Anomaly detectors based on Deep Neural Networks (DNNs) are the most frequently used method. However, some methods based on Graph Neural Networks (GNNs) have also been proposed recently. As a result, we evaluated both DNNs- and GNNs-based anomaly detectors. We used the following criteria to determine the baseline: 
    \begin{enumerate}[leftmargin=14pt]
        \item \textbf{\textit{Diverse Architecture}: } To ensure that we cover a broad range of methods, we decide that the baselines should be diverse, i.e., no two baselines have similar model architecture.
        \item \textbf{\textit{Diverse pre-processing}: } They should consider a different pre-processing technique (e.g., using raw data or feature vectors). 
        \item \textbf{\textit{Diverse post-processing}: } They should take into account various post-processing techniques for prediction (e.g., anomaly score, prediction error, or classification score). 
        \item \textbf{\textit{Peer-reviewed}: } The method is widely accepted and peer-reviewed. For this criterion, we take into account GitHub Forks, paper citations, and publication venues.
        \item \textbf{\textit{Open-source}: } The source code is freely available or can be obtained upon request.
    \end{enumerate}



    %(i)  (ii) (iii)  (iv)  (v)
    \subsubsection{\textbf{Selected Baselines}}
    We choose the following baselines based on the aforementioned criteria:%DNN based anomaly detectors are the most common methods. However, recently some Graph Neural Network based methods have also been proposed. Therefore, we considered DNNs as well as GNNs in our evaluation. For selecting the baseline we followed this criteria: (i) To cover a wide range of methods we decide that  selected baselines should be diverese i.e., no two baselines are similar in their model architecture. (ii) They should consider different types of pre-processing (e.g., using raw data or feature vectors). (iii) they should consider different post-processing for prediction (e.g., anomaly score, prediction error or classification score).  (iv) The method is peer-reviewed and widely adopted. We consider GitHub Forks, paper citations and publication venues for this criteria. (v) The code is openly available or available upon request. Based on these criterion, we selected the following baselines.
    
% \begin{itemize}[leftmargin=10pt]
    % \item
    \textbf{\textit{MSCRED} \citep{MSCRED} [\textit{AAAI'19}]: } Taking advantage of the temporal dependencies inherent in multivariate time series, \citet{MSCRED} proposed a Multi-Scale Convolutional Recurrent Encoder-Decoder (MSCRED) for anomaly detection on two datasets: (i) synthetic and (ii) power plant. Sidenote: \citet{OneClassNeurIPS} demonstrated that MSCRED outperforms all SOTA anomaly detection methods except Temporal Hierarchical One-Class (THOC), but we were unable to evaluate THOC as the code is not available (see more details below this list). As a result, we chose the second best method (i.e., MSCRED) among recently developed SOTA anomaly detection methods. Because the power plant dataset is not publicly available, we compare MSCRED with and without adversarial attack using the synthetic dataset used by \citet{MSCRED} in their work. 
    %Exploiting the temporal dependencies in multivariate time series X et al. proposed a Multi-Scale Convolutional Recurrent Encoder-Decoder (MSCRED) to perform anomaly detection on two datasets: (i) Synthetic and (ii) Power plant. Note: Shen et al. demonstrated that MSCRED outperforms all the SOTA anomaly detection methods except the Temporal Hierarchical One-Class (THOC), however we could not evaluate THOC as the code is not available (see more details below this list). Therefore, we selected the second best (i.e., MSCRED) among recent SOTA anomaly detection methods. The power plant dataset is not publicly available therefore we use the synthetic dataset used by X et al. in their work to provide a fair comparison of MSCRED with and without adversarial attack.
    
    % \item
    \textbf{\textit{CLMPPCA} \citep{CLMPPCA} [\textit{KDD'19}]: } \citet{CLMPPCA} proposed a hybrid approach for anomaly detection in multivariate satellite telemetry data. Based on the accomplishments of Convolutional LSTM-based networks in understanding spatiotemporal data in various domains~\cite{CONVLSTM_s1,CONVLSTM_s2,CONVLSTM_s4,CONVLSTM_s3}, they propose a Convolutional LSTM with Mixtures of Probabilistic Principal Component Analyzers (CLMPPCA) method for transforming the time window containing several telemetry data samples into a feature vector that is used to train the model and to predict the future data instances. To make final classification, the prediction errors calculated from the prediction and ground truth are combined with a moving average-based threshold method. In their work \citet{CLMPPCA} used a private dataset from the Korean Aerospace Research Institute's (KARI) KOMPSAT-5 satellite for evaluation. We were able to obtain the same private dataset and demonstrate how adversarial attacks affect the performance of CLMPPCA. One of the primary reasons for selecting CLMPPCA is that it is currently deployed at KARI. Thus, successfully demonstrating an attack on this method will demonstrate its applicability in a practical scenario.
    %Tariq et al. proposed hybrid approach to detect anomalies in a multivariate satellite telemetry data. They propose a Convolution LSTM with Mixtures of Probabilistic Principal Component Analyzers (CLMPPCA) method which transforms the past 10 minutes of telemetry data into a feature vector which is use to train the model and predict the future. The prediction errors calculate from the prediction and ground truth is used with a moving average based threshold method to make final classification. Tariq et al. used KOMPSAT-5 satellite's private dataset from Korean Aerospace Research Institute (KARI). We were able to acquire the same private dataset and demonstrate how the performance of CLMPPCA is impacted under adversarial attacks.
    
    % \item
    \textbf{\textit{MTAD-GAT} \citep{MTADGAT} [\textit{ICDM'20}]: } \citet{MTADGAT} proposed a multivariate time series anomaly detector based on Graph Attention Networks. The authors treat each univariate time series as a separate feature and employ two parallel graph attention layers to learn the complex dependencies between multivariate time series in both temporal and feature dimensions by jointly optimizing a forecasting-based and reconstruction-based model. MTAD-GAT outperformed several recent time series anomaly detectors such as OmniAnomaly~\citep{OmniAnomaly}, MAD-GAN~\citep{MADGAN}, and DAGMM~\citep{DAGMM} from ICLR 2018, on three publicly available anomaly datasets (SMAP, MSL, and SMD). As a result, MTAD-GAT is one of the best SOTA methods currently available. We evaluate MTAD-GAT with and without adversarial attacks on all three datasets (i.e., SMAP, MSL, and SMD). 
    %zhao et al proposed a Graph Attention Network based anomaly detector for multivariate time series. The authors considers each univariate time-series as an individual feature and includes two graph attention layers in parallel to learn the complex dependencies of multivariate time-series in both temporal and feature dimensions by jointly optimizes a forecasting-based model and a reconstruction-based model. MTAD-GAT showed state-of-the-art performance on three publicly available anomaly datasets (SMAP, MSL, SMD) beating several recent time-series anomaly detectors such as OmniAnomaly, MAD-GAN, DAGMM and more. This makes MTAD-GAT as one of the best among SOTA methods. We evaluate MTAD-GAT on all three datasets with and without adversarial attacks.
% \end{itemize}

\textbf{\textit{Note}:} We chose these three baselines based on their compliance with our defined criteria. Additionally, we were unable to evaluate some recent methods, such as Temporal Hierarchical One-Class (THOC) published at NeurIPS 2020 because the source code is not publicly available and our request to obtain the source code from the author was not answered. We discuss this further in Section~\ref{sec:repro}.
%Note that we selected these three baselines because they satisfied our defined criteria. Moreover, we could not evaluate some recent methods such as Temporal Hierarchical One-Class (THOC) published at NeurIPS 2020 because the code is not publicly available and our request to acquire the code from the author was not entertained.

\subsubsection{\textbf{White- and Black-box Attack Settings.} }
As the attacker will have complete knowledge of the underlying system in a White-box attack, we create attack vectors using the same selected baselines, namely MSCRED, CLMPPCA, and MTAD-GAT. Whereas for the Black-box attack, we build attack vectors using a model that is similar to but simpler than the victim model. For example, we utilise a vanilla recurrent autoencoder to create attack vectors for MSCRED, a simple CNN+LSTM model for CLMPPCA, and a vanilla GNN for MTAD-GAT.

\begin{comment}
\subsection{Intrusion Detection Baselines}
\label{sec:intrusion_baselines}
% \item \textit{Intrusion Detection Baselines}:
\cite{IntrusionSurvey} and \cite{IntrusionSurvey2} discuss the different domains where Intrusion detection-based methods are employed. We selected one such area, i.e., Intrusion detection in Vehicle Controller Area Network, and compared state-of-the-art solutions from this domain. We use the same criteria as anomaly detection to select the intrusion detection baselines as follows:

\begin{itemize}[leftmargin=10pt]
    \item \textbf{CAN-ADF. } \cite{CANADF} proposed a hybrid of heuristics and recurrent neural network (RNN) to detect different intrusions such as DoS, Fuzzing, and Replay attacks. The heuristics and RNN components in CAN-ADF complement each other resulting in significantly better performance and stability. The gradient-based attack can only be applied to the RNN component of CAN-ADF. Therefore, we believe it to be an interesting scenario where only one of the two components of the detector is attacked.
    \item \textbf{CANTransfer. } Recently, continual learning-based methods have become prevalent for intrusion detection. They can learn new intrusion signatures with only a few samples while keeping the same performance on previously learned intrusions. CANTransfer~\citep{CanTransfer} is one such method. The author first trains the base model on DoS Attack and then uses continual learning techniques to learn new intrusion such as Fuzzing and Replay by using only one attack instance. We believe that it will be interesting to observe the robustness of continual learning-based intrusion detectors against adversarial attacks.
\end{itemize}
Both CAN-ADF and CANTransfer use the same OTIDS dataset. Therefore, it gives us the opportunity to perform a fair comparison of two different systems (under adversarial attack) solving the same problem.
% \end{itemize}





% \Blindtext




% \begin{figure}
%     \centering
%     \includegraphics[trim={0pt 0pt 0pt 0pt},clip,width=1\linewidth]{figures/MSCRED.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \Blindtext

\end{comment}

==> sections/5_Results.tex <==
\section{Empirical Evaluation}
\label{sec:results}




We present results for the $\normmax$ FGSM and PGD attacks against three SOTA anomaly detection methods—MSCRED, CLMPPCA, and MTAD-GAT. %—as well as two controller area network intrusion detection methods—CAN-ADF and CANTransfer.
The Appendix includes additional details about the $\normmax$, $\normlone$, and $\normltwo$ attacks results (Appendix~\ref{app_sec:MSCRED}); % details on the $\normlone$ (Appendix~\ref{app_sec:L1}) and  (Appendix~\ref{app_sec:L2}) attacks;
more details on impact of adversarial attacks on MTAD-GAT (Appendix~\ref{app_sec:MTAD-GAT}); %(Appendix~\ref{app_sec:MTAD-GAT_MSL}--~\ref{app_sec:MTAD_SMD_Features};
some original vs. perturbed time series samples (Appendix~\ref{app_sec:CLMPPCA}. Moreover, results from the FGSM, PGD, BIM, Carlini-Wagner, and Momentum Iterative Method (MIM)~\citep{MIM} attacks on 71 datasets from the UCR repository are available on our GitHub repository. In general, we observe that perturbations that are $\normmax$-bounded are more effective. This could be explained by optimization challenges, as $\normlone$ and $\normltwo$ attacks are typically more difficult to optimize~\citep{CarliniWagnerL2,SL1D}.






 
\subsection{Adversarial Attack on MSCRED}
\subsubsection{\textbf{MSCRED (White-box)}}

We employ non-targeted FGSM and PGD methods to attack MSCRED. As a result, only $s_i$  from the test set is made available to the attack methods. The $\epsilon$ is set to $0.1$ for the FGSM attack, and $\alpha$ is set to $0.1$ for the PGD attack with $T=40$. The MSCRED method determines the appropriate threshold between normal and anomalous data points based on the training data. As a result, any modification to the test samples should not affect the threshold. As shown in Table~\ref{tab:mscred}, the victim model (MSCRED) has no efficacy on the samples perturbed by FGSM and PGD attacks and thus fails to detect all anomalies. Additionally, MSCRED classifies all instances of normal data as anomalies. We demonstrate in Figure~\ref{fig:mscred} that MSCRED (No Attack) can accurately predict the majority of anomalies with an F$_1$ score of $0.890$ (see Table~\ref{tab:mscred}). According to Figure~\ref{fig:mscred}, the anomaly scores under FGSM (yellow) and PGD (blue) attacks are always higher than the threshold (red dashed line), which means that MSCRED is predicting everything as an anomaly, resulting in an F$_1$ score of less than $0.50$.  It is intriguing that such a small amount of change in the time series, which is primarily imperceptible to the naked eye, can greatly affect the MSCRED's anomaly scores, even when the perturbations are so minute. The results in Table~\ref{tab:mscred} are demonstrating that MSCRED is not robust against adversarial attacks. 

\subsubsection{\textbf{MSCRED (Black-box)}} As with the White-box attack, the Black-box attack significantly reduced MSCRED's F1-score. This reduction, however, is slightly less than that caused by a White-box attack. Moreover, the PGD attack reduced F1-scores more than the FGSM attack, as shown in Table~\ref{tab:mscred}. This experiment demonstrates that even when we build the attack vector using a different backbone model, we can still achieve significant success by transferring the adversarial attack.


\subsection{Adversarial Attack on MTAD-GAT}
\subsubsection{\textbf{MTAD-GAT (White-box)}} As with MSCRED, we attack MTAD-GAT using a non-targeted FGSM and PGD method with $\epsilon=0.1$, $\alpha=0.1$, and $t = 40$. The results of adversarial attacks against MTAD-GAT trained on the MSL, SMAP, and SMD datasets are shown in Table~\ref{tab:mtad-gat}. MTAD-GAT demonstrates state-of-the-art performance for anomaly detection in the absence of an adversarial attack (No Attack). However, when adversarial examples from FGSM and PGD are used to evaluate it, the detection performance drops to as low as 66\%. The impact of the PGD attack is more significant than that of the FGSM attack, which is understandable given that PGD is a more powerful attack than FGSM. It leads us to ponder that if more sophisticated attacks are explicitly developed for time series data, they will have a significantly greater impact on SOTA anomaly detectors. As a result, future anomaly detection methods should take adversarial examples into account.

% \begin{table}[t]
%       \caption{MSCRED results (F$_1$ score) on synthetic dataset from original paper.}
%         \label{tab:mscred}
%         \vspace{-10pt}
%         \resizebox{0.7\linewidth}{!}{%
%         \begin{tabular}{lccc} 
%         \toprule
%         \textbf{Method~~~~~~~~~} & \textbf{Pre.} & \textbf{Rec.} & \textbf{F$_1$}\\
%         \hline
%         No Attack & 1.000 & 0.800 & 0.890 \\
%         FGSM & 0.487 & 0.500 & 0.493 \\
%         PGD & \textbf{0.485} & \textbf{0.500} & \textbf{0.492} \\
%         \bottomrule
%         \end{tabular}
%         % \vspace{10pt}
%         }
% \end{table}

% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
\centering
\caption{MSCRED results (F$_1$ score) on synthetic dataset from original paper. Both White- and Black-box attacks show significant success with FGSM and PGD. We used surrogate model (vanilla recurrent autoencoder) to generate adversarial examples for Black-box attack.}
\vspace{-10pt}
\label{tab:mscred}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc} 
\toprule
\multirow{3}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{White-box }} & \multicolumn{3}{c}{\textbf{Black-box }} \\
% & \multicolumn{3}{c|}{MSCRED} & \multicolumn{3}{c}{Vanilla Autoencoder} \\
 & \textit{\textbf{Pre.}} & \textit{\textbf{Rec.}} & \textit{\textbf{F$_1$}} & \textit{\textbf{Pre.}} & \textit{\textbf{Rec.}} & \textit{\textbf{F$_1$}} \\ 
\cline{2-7}
No Attack & 1.000 & 0.800 & 0.890  & 1.000 & 0.800 & 0.890  \\
FGSM & 0.487 & 0.500 & 0.493 & 0.651 & 0.693 & 0.671  \\
PGD & \textbf{0.485} & \textbf{0.500} & \textbf{0.492} & \textbf{0.634} & \textbf{0.677} & \textbf{0.655} \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table}

% \begin{table}[t]
%       \centering
%         \caption{MTAD-GAT results (F$_1$ score) on MSL, SMAP and SMD datasets.}
%         \label{tab:mtad-gat}
%         \vspace{-10pt}
%         \resizebox{0.84\linewidth}{!}{%
%         \begin{tabular}{lccc} 
%         \toprule
%         \textbf{Method} & \textbf{MSL} & \textbf{SMAP} & \textbf{SMD}\\
%         \hline
%         No Attack & 0.950 &	0.894 &	0.999 \\
%         FGSM & 0.719 & 0.804 & 0.803 \\
%         PGD & \textbf{0.687}	& \textbf{0.775} & \textbf{0.665} \\
%         \bottomrule
%         \end{tabular}
%         }
% \end{table}

% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
\centering
\caption{MTAD-GAT results (F$_1$ score) on MSL, SMAP and SMD datasets. For all three datasets, both White- and Black-box attacks are highly effective. We used vanilla GNN  as a surrogate model to generate adversarial examples for Black-box attack.}
\vspace{-10pt}
\label{tab:mtad-gat}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc} 
\toprule
\multirow{3}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{White-box}} & \multicolumn{3}{c}{\textbf{Black-box}} \\
%  & \multicolumn{3}{c|}{MTAD-GAT} & \multicolumn{3}{c}{Vanilla GNN} \\
 & \textbf{\textit{MSL}} & \textbf{\textit{SMAP}} & \textbf{\textit{SMD}} & \multicolumn{1}{c}{\textbf{\textit{MSL}}} & \multicolumn{1}{c}{\textbf{\textit{SMAP}}} & \multicolumn{1}{c}{\textbf{\textit{SMD}}} \\ 
\hline
No Attack & 0.950 & 0.894 & 0.999 & 0.950 & 0.894 & 0.999 \\
FGSM & 0.719 & 0.804 & 0.803 & 0.751 & 0.847 & 0.852 \\
PGD & \textbf{0.687} & \textbf{0.775} & \textbf{0.665} & \textbf{0.727} & \textbf{0.815} & \textbf{0.749} \\
\bottomrule
\end{tabular}
% }
\vspace{-10pt}
\end{table}



\begin{figure}[t!]
\centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[clip, trim=0pt 0pt 0pt 0pt,width=0.8\textwidth]{figures/MSCRED_3.pdf}
        \caption{No Attack, FGSM and PGD on MSCRED}
        \label{fig:mscred}
    \end{subfigure}\hfill
    % \vspace{10pt}
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[clip, trim=0pt 0pt 0pt 0pt,width=1\linewidth]{figures/MTAD.pdf}
        \caption{No Attack, FGSM and PGD on MTAD-GAT}
        \label{fig:mtad-gat}
    \end{subfigure}\hfill
    \vspace{-10pt}
    \caption{Anomaly score of No Attack, FGSM and PGD on MSCRED (a) and on MTAD-GAT for MSL dataset (b) The y-axis scale is between 0 and 1 for (b). See Appendix~\ref{app_sec:MSCRED} and ~\ref{app_sec:MTAD-GAT} for more details on (a) and (b), respectively.} 
    \label{fig:Results}
    \vspace{-10pt}
\end{figure}

% \begin{minipage}[t]{0.53\linewidth}
% % \begin{figure}

% % \end{figure}
%  \end{minipage}
% \hfill
% \begin{minipage}[t]{0.43\linewidth}

% % \begin{figure}
    
% % \end{figure}
% \end{minipage}

Additionally, Figure~\ref{fig:mtad-gat} illustrates the effect of adversarial examples from FGSM (yellow) and PGD (blue) attacks on the MTAD-GAT anomaly score for the MSL dataset.  We can see that the anomaly scores for FGSM and PGD frequently exceed the threshold (red dashed line), resulting in a large number of false positives and lowering the F$_1$ score from 94.98\% to 71.90\% for FGSM and 68.69\% for PGD.

\subsubsection{\textbf{MTAD-GAT (Black-box)}} Like the Black-box attack on MSCRED, the attack on MTAD-GAT has a similar effect, lowering the F1-score for MSL, SMAP, and SMD to 0.751, 0.847, and 0.852 with the FGSM attack and 0.727, 0.815, and 0.749 with the PGD attack, as shown in Table~\ref{tab:mtad-gat}. As with the Autoencoder, this experiment indicates that it is possible to transfer adversarial attack to graph neural networks. Thus, demonstrating that the adversary may not require extensive knowledge of the backbone to launch a successful attack.

\subsection{Adversarial Attack on CLMPPCA}
\subsubsection{\textbf{CLMPPCA (White-box)}} The KARI dataset is divided into ten subsystems. As a result, we trained the CLMPPCA model on each subsystem separately, as described in the original paper. We then used FGSM and PGD attacks to evaluate each of these trained models. For FGSM, we use $\epsilon=0.1$, for PGD, we use $\alpha=0.1$, and $t = 40$. Table~\ref{tab:clmppca} summarizes the prediction errors for each subsystem prior to and following the attack. We can see that when adversarial attacks are used, the prediction error increases up to twentyfold. Note: For brevity and space constraints, we omit the F$_1$ score from Table~\ref{tab:clmppca}, as it is $0.50$ for all subsystems. CLMPPCA fails to predict any anomalies under FGSM and PGD attacks because the prediction error is always higher than the threshold (see Figure~\ref{fig:clmppca}). We believe that by employing these straightforward yet effective attacks, an adversary can easily introduce false positives into CLMPPCA's predictions at will, posing significant difficulties for satellite operators.
%The KARI dataset contains 10 subsystems. Therefore, following the original paper, we trained the CLMPPCA model on each subsystem separately. We then evaluated each of these trained models with FGSM and PGD attack. We use $\epsilon=0.1$ for FGSM, $\alpha=0.1$, and $t = 40$ for PGD. In Table 4, we show the prediction errors before and after the attack for each subsystem. We can observe that the prediction error increase as much as twentyfolds under adversarial attacks. Under FGSM and PGD attack CLMPPCA fails to predict any anomalies as the prediction error always remain higher than the threshold (see Figure 1). Therefore, for the sake of brevity and due to lack of space we do not include the F1 score in Table 4 as it is 0.50 for all subsystem. Using these simple yet effective attacks the adversary can easily introduce false-positive into CLMPPCA's predictions at will.




% \begin{table*}[t]
% \centering
% \caption{CLMPPCA prediction errors on KARI KOMPSAT-5 dataset for subsystems (SS) 1-10.}
% \label{tab:clmppca}
% \vspace{-10pt}
% \resizebox{0.70\linewidth}{!}{%
% \begin{tabular}{lcccccccccc} 
% \toprule
% \textbf{Methods} & \textbf{SS1} & \textbf{\textbf{SS}2} & \textbf{\textbf{SS}3} & \textbf{\textbf{SS}4} & \textbf{\textbf{SS}5} & \textbf{\textbf{SS}6} & \textbf{\textbf{SS}7} & \textbf{\textbf{SS}8} & \textbf{\textbf{SS}9} & \textbf{\textbf{SS}10} \\ 
% \hline
% No Attack & 0.025 & 0.020 & 0.646 & 0.018 & 0.078 & 0.081 & 0.028 & 0.015 & 0.043 & 0.106 \\
% FGSM & 0.306 & 0.327 & 5.657 & 0.153 & 1.744 & 1.708 & 0.246 & 0.201 & 1.303 & 0.314 \\
% PGD & \textbf{0.688} & \textbf{0.748} & \textbf{11.200} & \textbf{0.205} & \textbf{2.459} & \textbf{3.391} & \textbf{0.430} & \textbf{0.231} & \textbf{1.798} & \textbf{0.555} \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

% \usepackage{graphicx}
% \usepackage{booktabs}


% \begin{table*}
% \centering
% \caption{CLMPPCA prediction errors for subsystems (SS) 1-10 on the KARI KOMPSAT-5 dataset from FGSM and PGD attack. The prediction errors enclosed in brackets are the result of Black-box attack, whereas those outside the brackets are from White-box attack. A higher error value indicates a more powerful attack. }
% \label{tab:clmppca}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccccccccc} 
% \toprule
% % \begin{tabular}[c]{@{}l@{}}\\\textbf{Methods}\end{tabular}

% \textbf{Methods} & \textbf{SS1} & \textbf{\textbf{SS}2} & \textbf{\textbf{SS}3} & \textbf{\textbf{SS}4} & \textbf{\textbf{SS}5} & \textbf{\textbf{SS}6} & \textbf{\textbf{SS}7} & \textbf{\textbf{SS}8} & \textbf{\textbf{SS}9} & \textbf{\textbf{SS}10} \\ 
% \hline
% No Attack & 0.025 & 0.020 & 0.646 & 0.018 & 0.078 & 0.081 & 0.028 & 0.015 & 0.043 & 0.106 \\
% FGSM & 0.306 (0.132) & 0.327 (0.159) & 5.657 (3.163) & 0.153 (0.092) & 1.744 (0.680) & 1.708 (0.616) & 0.246 (0.115) & 0.201 (0.098) & 1.303 (0.724) & 0.314 (0.191) \\
% PGD & \textbf{0.688 (0.333)} & \textbf{0.748 (0.382)} & \textbf{11.20 (5.216)} & \textbf{0.205 (0.135)} & \textbf{2.459 (1.301)} & \textbf{3.391 (1.630)} & \textbf{0.430 (0.206)} & \textbf{0.231 (0.139)} & \textbf{1.798 (1.105)} & \textbf{0.555 (0.249)} \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}
% \usepackage{graphicx}
% \usepackage{booktabs}


\begin{table*}
\centering
\caption{CLMPPCA prediction errors for subsystems (SS) 1-10 on the KARI KOMPSAT-5 dataset from FGSM and PGD attack. The prediction errors enclosed in brackets are the result of Black-box attack, whereas those outside the brackets are from White-box attack. A higher error value indicates a more powerful attack.}
\vspace{-10pt}
\label{tab:clmppca}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccccccccc} 
\toprule
% \begin{tabular}[c]{@{}l@{}}\\\textbf{Methods}\end{tabular}
\textbf{Methods} & \textbf{SS1} & \textbf{\textbf{SS}2} & \textbf{\textbf{SS}3} & \textbf{\textbf{SS}4} & \textbf{\textbf{SS}5} & \textbf{\textbf{SS}6} & \textbf{\textbf{SS}7} & \textbf{\textbf{SS}8} & \textbf{\textbf{SS}9} & \textbf{\textbf{SS}10} \\ 
\hline
No Attack & 0.025 & 0.020 & 0.646 & 0.018 & 0.078 & 0.081 & 0.028 & 0.015 & 0.043 & 0.106 \\ 
\hline
\multirow{2}{*}{FGSM } & 0.306 & 0.327 & 5.657 & 0.153 & 1.744 & 1.708 & 0.246 & 0.201 & 1.303 & 0.314 \\
 & \multicolumn{1}{l}{(0.132)} & \multicolumn{1}{l}{(0.159)} & \multicolumn{1}{l}{(3.163)} & \multicolumn{1}{l}{(0.092)} & \multicolumn{1}{l}{(0.680)} & \multicolumn{1}{l}{(0.616)} & \multicolumn{1}{l}{(0.115)} & \multicolumn{1}{l}{(0.098)} & \multicolumn{1}{l}{(0.724)} & \multicolumn{1}{l}{(0.191)} \\ 
\hline
\multirow{2}{*}{PGD} & \textbf{0.688} & \textbf{0.748} & \textbf{11.20} & \textbf{0.205} & \textbf{2.459} & \textbf{3.391} & \textbf{0.430} & \textbf{0.231} & \textbf{1.798} & \textbf{0.555} \\
 & \multicolumn{1}{l}{\textbf{\textbf{(0.333)}}} & \multicolumn{1}{l}{\textbf{\textbf{(0.382)}}} & \multicolumn{1}{l}{\textbf{\textbf{(5.216)}}} & \multicolumn{1}{l}{\textbf{\textbf{(0.135)}}} & \multicolumn{1}{l}{\textbf{\textbf{(1.301)}}} & \multicolumn{1}{l}{\textbf{\textbf{(1.630)}}} & \multicolumn{1}{l}{\textbf{\textbf{(0.206)}}} & \multicolumn{1}{l}{\textbf{\textbf{(0.139)}}} & \multicolumn{1}{l}{\textbf{\textbf{(1.105)}}} & \multicolumn{1}{l}{\textbf{\textbf{(0.249)}}} \\
\bottomrule
\end{tabular}
% }
\vspace{-10pt}
\end{table*}

\subsubsection{\textbf{CLMPPCA (Black-box)}} We generated the attack vector using a CNN$+$LSTM surrogate model and evaluated the CLMPPCA model in a Black-box scenario. As with the other two Black-box experiments (i.e., MSCRED and MTAD-GAT), we saw a similar trend. The CLMPPCA model's prediction error does increase consistently for all subsystems when the attack vector is constructed using the surrogate model, as shown in Table~\ref{tab:clmppca}; in round brackets.
We can deduce from the CLMPPCA Black-box results that all three types of models investigated in this work (i.e., Autoencoder, DNNs, GNNs) are relatively equally susceptible to transferable adversarial attacks via surrogate models.

\subsection{\textbf{Summary of Results}}
Our findings indicate that the majority of SOTA anomaly detectors prioritized performance over robustness. This could have dire consequences if such systems are deployed in real-world systems. CLMPPCA is one such example, which is currently being deployed at KARI. Please note that we have informed KARI of the vulnerability in CLMPPCA; additional information is available in our Ethics Statement (see Section~\ref{sec:ethics}). Additionally, leveraging a surrogate model to conduct a Black-box attack can have a severe effect on the performance of the victim model. However, there are several limitations to surrogate, which we shall discuss in Section~\ref{sec:limitations}.


\begin{comment}
\subsection{Adversarial Attack on CAN Intrusion Detectors}


We evaluate the robustness of two popular and recent Controller Area Network intrusion detectors under adversarial impact. We use the same experimental settings (i.e., same training and test sets, $epochs=50$) and attack settings (i.e., $\epsilon=0.1$, $\alpha=0.1$ and $T=40$) for CAN-ADF and CANTransfer to have a fair comparison.



\textbf{CAN-ADF Performance. } 
The results for CAN-ADF under no attack, FGSM attack, and PGD attack are presented in Table~\ref{tab:intrusion}, column 2. While CAN-ADF outperforms CANTransfer in a normal scenario (i.e., no attack), it is also more vulnerable to adversarial attacks, with an F$_1$ score of $0.00$ for the PGD attack. Even though we could only attack the RNN component of CAN-ADF and the heuristics component remained unaffected, CAN-ADF's poor performance against adversarial attacks demonstrates its high reliance on the RNN component.

\begin{table}
\centering
\caption{CAN-ADF and CANTransfer results (F$_1$ score) on OTIDS dataset.}
\label{tab:intrusion}
% \vspace{-10pt}
\resizebox{0.84\linewidth}{!}{%
\begin{tabular}{lcc} 
\toprule
\textbf{Method} & \textbf{CAN-ADF} & \textbf{CANTransfer} \\ 
\hline
No Attack & 0.987 & 0.879 \\
FGSM & 0.188 & 0.858 \\
PGD & \textbf{0.000} & \textbf{0.311} \\
\bottomrule
\end{tabular}
}
\end{table} 

% \end{table}


\textbf{CANTransfer Performance. } Table~\ref{tab:intrusion}, column 3 contains the results for CANTransfer with no attack, FGSM attack, and PGD attack. While CANTransfer performs slightly worse than CAN-ADF in the absence of an attack ($0.879$), it exhibits greater resistance to adversarial attacks than CAN-ADF, particularly against FGSM attacks, where CANTransfer's performance drops by only $2\%$. We attempted multiple runs of the experiment, but the results remained consistent for the FGSM attack. Under PGD, it is a different tale, as CANTransfer's performance drops significantly from $0.879$ to $0.311$, demonstrating its vulnerability.

These findings demonstrate that neither of the two most recent intrusion detectors for Controller Area Networks is resistant to adversarial examples. As a result, future research should consider the robustness of new detectors against adversarial attacks when designing them.

\end{comment}


